HDOT -- an Approach Towards Productive Programming of Hybrid Applications

MPI applications matter. However, with the advent of many-core processors, traditional MPI applications are challenged to achieve satisfactory performance. This is due to the inability of these applications to respond to load imbalances, to reduce serialization imposed by synchronous communication patterns, to overlap communication with computation and finally to deal with increasing memory overheads. The MPI specification provides asynchronous calls to mitigate some of these factors. However, application developers rarely make the effort to apply them efficiently. In this work, we present a methodology to develop hybrid applications called Hierarchical Domain Over-decomposition with Tasking (HDOT), that reduces programming effort by emphasizing the reuse of data partition schemes from process-level and applying them on task-level, allowing a top-down approach to express concurrency and allowing a natural coexistence between MPI and shared-memory programming models. Our integration of MPI and OmpSs-2 shows promising results in terms of programmability and performance measured on a set of applications.

==> tex/halos.tex <==
Data structures found on typical HPC applications, e.g.\ those relying on stencil operations, are artificially increased with halos (also called ghost points).  Such halos are indeed memory copies from neighbour MPI processes that need to be constantly communicated via point-to-point MPI calls.  A pure MPI application gets its parallelism by increasing the number of MPI domains (or ranks) and, as a consequence, there is (i) an increase of allocated memory for halos followed by (ii) an increase of information that needs to be communicated between ranks.

For data structures corresponding to simple geometries\footnote{In 1D a line of $N_{lg}$ elements, in 2D a square of $N_{lg}^2$ elements and, in 3D, a cube of $N_{lg}^3$ elements where $N_{lg}$ is the characteristic number of elements of the local grid (per MPI domain) without halos.}, like those typically found on matrix-multiplication algorithms or Finite Difference Method (FDM) based applications, the ratio between the allocated memory assigned to halos and the memory allocated for the local grid (per MPI domain) is given by $r_{h/lg} = (2N_hN_{lg}^{D-1}D +2^{D-1}N_h^D(D-1))/N_{lg}^D$ where $N_h$ is the characteristic number of halo elements and $D$ the grid dimension.  It can be readily seen in Figure~\ref{fig:memoryRatio} that this ratio can reach values up to 100\% for moderate local grid sizes if the number of halo elements $N_h$ increases (e.g.\ see red solid line).  Moreover, for 2D and 3D problems it is often necessary to perform MPI communication in more than one direction (the MPI domain cuts are contiguous in memory only for one direction) to exploit parallelism, which further increases this ratio: from 20\% for 1D MPI decomposition up to 60.8\% for 3D MPI decomposition for $N_{h}/N_{lg}=0.1$.

%
\begin{figure}[tp]
%
  \begin{minipage}[c]{0.49\textwidth}
    \begin{center}
      \subfloat[]{
        \includegraphics[width=0.98\textwidth]{./pics/pdf/memoryRatio}\label{fig:memoryRatio}
      }
    \end{center}
  \end{minipage}
  %
  \begin{minipage}[c]{0.49\textwidth}
    \begin{center}
      \subfloat[]{
        \includegraphics[width=0.98\textwidth]{./pics/pdf/messageSize}\label{fig:messageSize}
      }
      \end{center}
  \end{minipage}
%
  \caption{(a) Halo to local grid memory ratio ($r_{h/lg}$) as a function of the characteristic halo size ($N_h$) and characteristic local grid size ($N_{lg}$) and (b) non-dimensional amount of information exchanged via MPI ($M^*$) as a function of the number of shared-memory processes ($N_{sp}$), distributed-memory processes ($N_{dp}$) and total number of processes ($N_{tp} = N_{sp} \times N_{dp}$).  A grid with notation $\alpha$D-$\beta$ has $\alpha$ spatial dimensions and is decomposed in $\beta$ dimensions for MPI communication.}
%
  \label{fig:memoryRatio-messageSize}
%
\end{figure}
%

Figure~\ref{fig:messageSize} shows the \emph{non-dimensional} amount of information exchanged via MPI messages $M^*$ as a function of the number of shared- and distributed-memory processes, $N_{sp}$ and $N_{dp}$, respectively.  It is worth mentioning that the \emph{actual} amount of communicated data increases significantly with the grid dimension, total number of grid elements and the halo size\footnote{The actual amount of information exchanged is calculated as $M=M^* \times M_{\mathrm{ref}}$ where $M_{\mathrm{ref}}=2N_dN_hN_g^{D-1}$, $N_d$ is the amount of data (e.g.\ floats) contained in a single element of the halo and $N_g$ is the characteristic number of elements of the whole grid (e.g.\ a cubic grid has $N_g^3$ elements).}.  However, the non-dimensional notation allow us to simplify this study using a single equation, $M^*=D(\sqrt[D]{N_{tp}/N_{sp}} -1)$, that can be applied to 1D, 2D and 3D data structures.  The value of $M^*$ increases proportionally to the dimensions of the grid and the $D$-root of the number of distributed-memory processes $N_{dp} = N_{tp} / N_{sp}$.  Consequently, MPI communication in more than one dimension, although can have a significant increase in memory due to presence of more halos %FIXME is this sentence true?
, do reduce the overall amount of information to be exchanged: this is indeed most noticeable for 2D communication.  Also as expected, pure MPI applications (see the plane $N_{sp}=1$ in Figure~\ref{fig:messageSize}) need to communicate the largest amount of data and, increasing the number of shared-memory processes whilst keeping the total number of processes constant (i.e.\ a hybrid approach) has the benefit of diminishing this data (e.g.\ see red curve).


